Aligning Pre-trained Models for Spoken Language Translation

This paper investigates a novel approach to end-to-end speech translation (ST) based on aligning frozen pre-trained automatic speech recognition (ASR) and machine translation (MT) models via a small connector module (Q-Former, our Subsampler-Transformer Encoder). This connector bridges the gap between the speech and text modalities, transforming ASR encoder embeddings into the latent representation space of the MT encoder while being the only part of the system optimized during training. Experiments are conducted on the How2 English-Portuguese dataset as we investigate the alignment approach in a small-scale scenario focusing on ST. While keeping the size of the connector module constant and small in comparison ( < 5% of the size of the larger aligned models), increasing the size and capability of the foundation ASR and MT models universally improves translation results. We also find that the connectors can serve as domain adapters for the foundation MT models, significantly improving translation performance in the aligned ST setting. We conclude that this approach represents a viable and scalable approach to training end-to-end ST systems.

==> tikz_old.tex <==
\begin{figure}[h]
    \centering
    \begin{tikzpicture}[
    asrnode/.style={rectangle, draw=blue!20!black, fill=blue!20, rounded corners=5, very thick, minimum height=10mm, minimum width=25mm},
    mtnode/.style={rectangle, draw=blue!20!black, fill=blue!20, rounded corners=5, very thick, minimum height=10mm, minimum width=25mm},
    connector/.style={rectangle, draw=red!20!black, fill=red!20, rounded corners=5, very thick, minimum height=10mm},
    box/.style={rectangle, draw=black, very thick},
    arrow/.style = {thick, ->, >=stealth}
    ]
    
      % Define the number of rectangles
      %\def\n{5}
      %% Define the width and height of each rectangle
      %\def\rectwidth{0.2}
      %\def\rectheight{1}
      
      % Loop to draw the rectangles
      %\foreach \i in {0,...,\n} {
      %  \draw[fill=yellow] (\i * \rectwidth * 1.4, 0) rectangle ++(\rectwidth, \rectheight);
      %}
    
      \node[asrnode] (ASRenc)                  {ASR encoder};
      \node[connector] (Connector)            [above=0.5 of ASRenc]          {Connector};
      \node[box] (Concat)              [above=1.2 of Connector]          {Concat.};
      \node[mtnode] (MTenc)            [above=0.3 of Concat]          {MT encoder};
      \node[box] (Prompt)              [above left=0.2 of Connector, xshift=8mm]          {\scriptsize{\texttt{`translate: `}}}
      \node[mtnode] (MTdec)            [above=0.5 of MTenc]          {MT decoder};
      \node[] (X) [below=0.5 of ASRenc] {$\mathbf{x}$};
      \node[] (Y) [above=0.5 of MTdec] {$L_{\text{CE}}(\mathbf{y, z})$};
    
      \draw[arrow] (X) -- (ASRenc.south);
      \draw[arrow] (ASRenc.north) -- (Connector.south);
      \draw[arrow] (Connector.north) .. controls +(0mm,5mm) and +(0mm,-5mm) .. ([xshift=2mm]Concat.south);
      \draw[arrow] (Prompt.north) .. controls +(0mm,3mm) and +(0mm,-5mm) .. ([xshift=-2mm]Concat.south);
      \draw[arrow] (Concat.north) -- (MTenc.south);
      \draw[arrow] (MTenc.north) to node[right] {\scriptsize{\texttt{C/A}}} (MTdec.south);
      \draw[arrow] (MTdec.north) -- (Y);
      
      \node[asrnode] (ASRenc2)        [right= 10mm of ASRenc]        {ASR encoder};
      \node[connector] (Connector2)            [above=0.5 of ASRenc2]          {Connector};
      \node[mtnode] (MTdec2)            [above=of Connector2, right=of MTdec]          {MT decoder};
      \node[] (X2) [below=0.5 of ASRenc2] {$\mathbf{x}$};
      \node[] (Y2) [above=0.5 of MTdec2] {$L_{\text{CE}}(\mathbf{y, z})$};
    %
      \draw[arrow] (X2) -- (ASRenc2.south);
      \draw[arrow] (ASRenc2.north) -- (Connector2.south);
      \draw[arrow] (Connector2.north) to node[right] {\scriptsize{\texttt{C/A}}} (MTdec2.south);
      \draw[arrow] (MTdec2.north) -- (Y2);

      \node[] (A) [below=0.3 of X] {\large{ECED}}
      \node[] (B) [below=0.3 of X2] {\large{ECD}}

    \end{tikzpicture}
    \caption{\todo{I don't like this, rework, rewrite, alter the digaram?}Diagram of the ECED (left) and ECD (right) alignment architectures, where $\mathbf{x}$ denotes the input speech utterance, \mathbf{}. For the ECED architecture, the connector output embeddings can be concatenated with the text embeddings of a text prompt for the MT encoder.}
    \label{fig:enter-label}
\end{figure}
